On the Dark Matter Halos of Optical and IR-selected AGN in the Local Universe

We use the technique of total satellite luminosity, L_sat, to probe the dark matter halos around active galactic nuclei in the SDSS Main Galaxy Sample. Our results focus on galaxies and AGN that are the central galaxy of their halo. Our two AGN samples are constructed from optical emission-line diagnostics and from WISE infrared colors. Both optically-selected and WISE-selected AGN have L_sat values twice as high as non-active galaxy samples when controlling for stellar mass and mean stellar age. This implies that the halos are twice as massive, but we cannot rule out that the increase in L_sat is due to these AGN residing in younger halos at the same mass. When only controlling for host galaxy stellar mass, WISE-selected AGN also have higher L_sat values than optical AGN at the factor of two level, consistent with previous results comparing the clustering of obscured and unobscured AGN. However, controlling for stellar age in the two populations of host galaxies removes half of this difference, attenuating the statistical significance of the difference. We perform permutation tests to quantify the different in the halo populations of each sample. The difference in star formation properties does not fully explain the difference in the two AGN populations, however. Although AGN luminosity correlates with mean stellar age, the difference in stellar age between the WISE and optical samples cannot be fully explained by differences in their AGN luminosity distributions.

==> overflow.tex <==
The $\lsat$ measurements demonstrate that dust-obscured AGN occupy
different halos than optical AGN. Combined with the results of
clustering studies of quasars that demonstrate higher clustering
amplitude of obscured QSOs relative to optical samples, this implies
that the difference in $\lsat$ is due to changes in $\mhalo$ as
opposed to changes in halo formation history. At the peak of the
$\mgal$ distribution, $10^{10.6}$ $\msol$, the mean halo mass is
$\sim 10^{12.0}$ $\hmsol$ (cf., the compilation of SHMR results in
Figure 2 of \cite{wechsler_tinker:18}). At this halo mass scale,
$\lsat$ corresponds nearly linearly to $\mhalo$.  Thus, the $\chibar$
results from Figure \ref{lsatbar} imply halo masses for the two AGN
samples of $\log M_{\rm obs}=12.38\pm 0.11$ and
$\log M_{\rm opt}= 12.11 \pm 0.04$. The difference between the two
halo masses, $0.27 \pm 0.12$ dex, is consistent within 1$\sigma$ with
the results of \cite{dipompeo_etal:17} who find
$\Delta \log \mhalo = 0.45 \pm 0.13$ dex. The halo masses themselves
are $\sim 0.5$ dex lower than those found in \cite{dipompeo_etal:17},
but we note that the sample selections are markedly different both in
terms of the redshift and the luminosity---DiPompeo use photometric
samples of bright quasars at $z\sim 1$. Our samples are more
comparable to that of \cite{mendez_etal:16}, who analyze lower
luminosity spectroscopic samples at $z\sim 0.7$. \cite{mendez_etal:16}
find much {\it lower} halo masses than in this work, but we again note
that the small sample size and resulting errors in halo mass make the
statistical difference minimal.


%----

\cite{dipompeo_etal:17_model} propose an empirical model to explain
the difference in halo masses. In this model, during the quiescent
phase with no nuclear activity and thus no black hole growth, BHs will
fall below the mean relation BH-$\mhalo$ relation. When this occurs,
the BHs become active, first with a dust-obscured phase, and then with
an optical phase after the BHs have grown some amount. At fixed halo
mass, then, obscured AGN have less massive BHs than
unobscured. At fixed BH mass, however, AGN in the obscured phase live
in more massive halos.

In this work, we are also able to bring the stellar mass of the host
central galaxy into the fold. At fixed $\lsat$---and, by extension,
fixed $\mhalo$--- there is a clear sequence in $\mgal$ and star
formation properties. WISE-AGN have the lowest stellar masses, but the
highest star formation rates; BPT-AGN have intermediate values of both
$\mgal$ and SFR, while halos with non-active galaxies have the highest
stellar masses and lowest fraction of galaxies on the star-forming
sequence. If BH growth and stellar growth are correlated, with respect
to their mean relations with $\mhalo$, then the scenario outlined in
\cite{dipompeo_etal:17_model} is consistent with the results presented
here.


